PELMS: Pre-training for Effective Low-Shot Multi-Document Summarization

We investigate pre-training techniques for abstractive multi-document summarization (MDS), which is much less studied than summarizing single documents. Though recent work has demonstrated the effectiveness of highlighting information salience for pre-training strategy design, it struggles to generate abstractive and reflective summaries, which are critical properties for MDS. To this end, we present PELMS, a pre-trained model that uses objectives based on semantic coherence heuristics and faithfulness constraints with un-labeled multi-document inputs, to promote the generation of concise, fluent, and faithful summaries. To support the training of PELMS, we compile MultiPT, a multi-document pre-training corpus containing over 93 million documents to form more than 3 million unlabeled topic-centric document clusters, covering diverse genres such as product reviews, news, and general knowledge. We perform extensive evaluation of PELMS in low-shot settings on a wide range of MDS datasets. Our approach consistently outperforms competitive comparisons with respect to overall informativeness, abstractiveness, coherence, and faithfulness.

==> tables/primary_results_zero_shot.tex <==
\begin{tabular}{lcccclcccclcccc}
\hline
                               & \multicolumn{4}{c}{Amazon}                                    &  & \multicolumn{4}{c}{Duc2004}                                  &  & \multicolumn{4}{c}{MetaTomatoes}                             \\ \hline
\multicolumn{1}{l|}{}          & R1            & R2            & RL            & RG            &  & R1            & R2           & RL            & RG            &  & R1            & R2           & RL            & RG            \\ \cline{2-15} 
\multicolumn{1}{l|}{Pegasus-X} & 25.9          & 4.2           & 15.1          & 11.8          &  & 31.3          & 5.5          & 15.6          & 13.9          &  & 29.6          & 4.4          & 13.5          & 12.0          \\
\multicolumn{1}{l|}{Primera}   & 29.4          & 5.4           & 16.5          & 13.8          &  & \textbf{34.8} & \textbf{7.6} & \textbf{18.3} & \textbf{16.9} &  & 28.4          & 4.5          & 13.5          & 12.0          \\
\multicolumn{1}{l|}{PELMS}     & \textbf{35.3} & \textbf{7.7}  & \textbf{21.6} & \textbf{18.1} &  & 32.7          & 6.7          & 16.9          & 15.5          &  & \textbf{33.5} & \textbf{6.9} & \textbf{16.0} & \textbf{15.5} \\ \hline
                               & \multicolumn{4}{c}{MultiNews}                                 &  & \multicolumn{4}{c}{Multi-X-Science}                          &  & \multicolumn{4}{c}{Yelp}                                     \\ \hline
\multicolumn{1}{l|}{}          & R1            & R2            & RL            & RG            &  & R1            & R2           & RL            & RG            &  & R1            & R2           & RL            & RG            \\ \cline{2-15} 
\multicolumn{1}{l|}{Pegasus-X} & 25.3          & 7.6           & 13.7          & 13.8          &  & 23.1          & 3.4          & 13.3          & 10.1          &  & 21.8          & 2.8          & 13.6          & 9.4           \\
\multicolumn{1}{l|}{Primera}   & 39.5          & 11.9          & 18.8          & 20.7          &  & 27.9          & 4.4          & \textbf{15.1} & 12.3          &  & 25.8          & 3.9          & 15.5          & 11.6          \\
\multicolumn{1}{l|}{PELMS}     & \textbf{43.1} & \textbf{14.4} & \textbf{20.9} & \textbf{23.5} &  & \textbf{28.9} & \textbf{4.6} & 14.9          & \textbf{12.6} &  & \textbf{30.5} & \textbf{6.2} & \textbf{18.3} & \textbf{15.1} \\ \hline
\end{tabular}
